Logistic-Regression with peer-group effects via inference in higher order Ising models

Spin glass models, such as the Sherrington-Kirkpatrick, Hopfield and Ising models, are all well-studied members of the exponential family of discrete distributions, and have been influential in a number of application domains where they are used to model correlation phenomena on networks. Conventionally these models have quadratic sufficient statistics and consequently capture correlations arising from pairwise interactions. In this work we study extensions of these to models with higher-order sufficient statistics, modeling behavior on a social network with peer-group effects. In particular, we model binary outcomes on a network as a higher-order spin glass, where the behavior of an individual depends on a linear function of their own vector of covariates and some polynomial function of the behavior of others, capturing peer-group effects. Using a {\em single}, high-dimensional sample from such model our goal is to recover the coefficients of the linear function as well as the strength of the peer-group effects. The heart of our result is a novel approach for showing strong concavity of the log pseudo-likelihood of the model, implying statistical error rate of $\sqrt{d/n}$ for the Maximum Pseudo-Likelihood Estimator (MPLE), where $d$ is the dimensionality of the covariate vectors and $n$ is the size of the network (number of nodes). Our model generalizes vanilla logistic regression as well as the peer-effect models studied in recent works, and our results extend these results to accommodate higher-order interactions.

==> intro_backup_costis.tex <==
\section{Introduction}
\label{sec:intro}

Did you choose \textcolor{red}{red} rather than \textcolor{blue}{blue} because some inherent attributes of yours biased you towards \textcolor{red}{red}, or because your social environment biased you towards that color? Of course, the answer is typically ``\textcolor{red}{bo}\textcolor{blue}{th}.'' Indeed, a long literature in econometrics and the social sciences has substantiated the importance of peer effects in network behavior in topics as diverse as criminal activity (see e.g.~\cite{glaeser1996crime}), welfare participation (see e.g.~\cite{bertrand2000network}), school achievement (see e.g.~\cite{sacerdote2001peer}), participation in retirement plans (see e.g.~\cite{duflo2003role}), and obesity (see e.g.~\cite{trogdon2008peer,christakis2013social}).
%A prominent dataset where peer effects have been studied are data collected by the National Longitudinal Study of Adolescent Health, a.k.a.~AddHealth study~\cite{harris2009waves}. This was a major national study of students in grades 7-12, who were asked to name their friends---up to 10, so that friendship networks can be constructed, and answer hundreds of questions about their personal and school life, and it also recorded information such as the age, gender, race, socio-economic background, and health of the students.
Estimating models incorporating peer and individual effects as drivers of behavior in such settings has been challenging; see~e.g.~\cite{manski1993identification,bramoulle2009identification}.

From a modeling perspective, a class of probabilistic models that are commonly used to model binary behavior in social networks are spin glass models, such as the well-studied Sherrington-Kirkpatrick, Hopfield and Ising models. In these models, a vector of binary behaviors $\vec{y} \in \{-1,1\}^V$ across all nodes of some network $G=(V,E)$ is sampled jointly according to the Gibbs distribution, $p(\vec{y})={1 \over Z} \exp(-{\rm En}(\vec{y}))$, defined by some energy function ${\rm En}(\vec{y})$ of the aggregate behavior, where the functional form of ${\rm En}(\cdot)$ typically depends on characteristics of the nodes as well as the structure of their social network. Such models studied originally in Statistical Physics, have found myriad applications in diverse fields, including probability theory, Markov Chain Monte Carlo, Computer Vision, Computational Biology,  Game Theory, and, related to our focus, Economics and the Social Sciences~\cite{LevinPW09,Chatterjee05,Felsenstein04,DaskalakisMR11,GemanG86,Ellison93,MontanariS10}.

Closely related to our work, a series of recent works have studied estimation of spin glass models incorporating both peer and individual effects as drivers of behavior~\cite{Chatterjee07,ghosal2018joint,DDP19}. Generalizing the classical logistic regression model, these works consider models of binary behavior on a  network, conforming to the following general class of models. Suppose that the nodes of a social network $G=(V,E)$ have individual characteristics $\vec{x}_i \in \mathbb{R}^d$, $i \in V$, and sample binary behaviors $\vec{y} \in \{\pm 1\}^V$ according to some measure that combines individual and peer effects, taking the following form:
\begin{align}\Pr[\vec{y}] = {1 \over Z_{\theta,\beta}} \exp\left(\sum_{i=1}^n(\theta^{\rm T} \vec{x}_i) y_i + \beta\cdot f(\vec{y})\right), \label{eq:the model}
\end{align}
where a linear function $\theta^T \vec{x}_i$ of node $i$'s individual characteristics determines the ``external field'' on that node, i.e.~the direction and strength of the ``local push'' of that node towards $-1$ or $+1$, and some function $f(\vec{y})$ of the nodes' joint behavior expresses what configurations in $\{\pm 1 \}^V$ are encouraged by peer-group effects. In particular, setting $\beta=0$ recovers the standard logistic regression model, where nodes choose their behaviors independently, but setting $\beta>0$ incorporates peer-group effects, as expressed by $f$. Without loss of generality, $f$ is a multi-linear function, and we can take $E$ to contain a hyperedge for each monomial in $f$, i.e.~take $f(\vec{y})=\sum_{\vec{e} \in E} w_{\vec{e}} \vec{y}_{\vec{e}}$.

Given a collection $\vec{x}_1,\ldots,\vec{x}_n \in \mathbb{R}^d$ of covariates, some function $f: \{\pm 1\}^V \rightarrow \mathbb{R}$, and a {\em single} sample $\vec{y}$  drawn from a model conforming to~\eqref{eq:the model}, the afore-cited works of Chatterjee~\cite{Chatterjee07}, Ghosal and Mukerjee~\cite{ghosal2018joint} and Daskalakis et al.~\cite{DDP19} provide computationally and statistically efficient algorithms for estimating $\theta$ and $\beta$. Specifically, these works study the restriction of model~\eqref{eq:the model} to the case where $f$ contains only pair-wise effects, i.e.~where function $f$ is a multilinear function of degree $2$. In particular, Chatterjee~\cite{Chatterjee07} studies the case where $\theta=0$ and $f$ is bilinear, Ghosal and Mukerjee~\cite{ghosal2018joint} the case where $d=1$, all $x_i$'s equal $1$, and $f$ is bilinear, while Daskalakis et al.~\cite{DDP19}  the general bilinear case. Extending these works, the goal of our work is to provide computationally and statistically efficient estimation methods for models where $f$ has peer effects of higher-order. As such, our new methods can accommodate richer models, capturing a much broader range of social interactions, e.g.~settings where nodes belong in various groups, and dislike fragile majorities in the groups they belong to. Our main result is the following.
%
 %drawn according to measure~\eqref{eq:the model}, our goal is to output an estimate $(\hat{\theta},\hat{\beta})$ of the true parameters $(\theta,\beta)$. 

\begin{theorem}[Informal] \label{thm:informalone}
Let $G=(V,E,w:E \rightarrow \mathbb{R})$ be a weighted hypergraph with edges of cardinality at least two and at most $m$, and let $f(\vec{y})=\sum_{\vec{e} \in E} w_{\vec{e}} \vec{y}_{\vec{e}}$. Assume that each vertex has bounded degree (Assumption \ref{eq:bounded}) and the hypergraph is dense enough (Assumption \ref{eq:lowebounded}). Moreover, assume that true parameters $\theta_0, \beta_0$ and the feature vectors have bounded $\ell_2$ norm, and the empirical covariance matrix of the feature vectors has singular values upper and lower bounded by constants (Assumption \ref{eq:assumption3}). Then, there exists a polynomial-time algorithm, which, given a single sample from model~\eqref{eq:the model}, outputs an estimate $(\tilde{\theta}, \tilde{\beta})$ such that $\norm{(\tilde{\theta},\tilde{\beta})-(\theta_0,\beta_0)}_2 \le 2^{O(m)} \cdot O\left(\sqrt{\frac{d}{n}}\right)$, with probability at least $99\%$.
\end{theorem}

\paragraph{Discussion of Main Result.} First, let us discuss the assumptions made in our statement. Note that the assumptions about $\theta$ and the $x_i$'s are standard, and are commonly made even for vanilla logistic regression without peer effects ($\beta=0$). The assumption about the boundedness of $\beta$ and the degree of the hypergraph is needed so that the peer-group effects do not overwhelm the individual effects, making $\theta$ non-identifiable. Finally, the assumption on the density of the hypergraph is needed so that the individual effects do not overwhelm the peer-group effects, making $\beta$ non-identifiable. Our assumptions about $\beta$ and the hypergraph are generalizations of corresponding assumptions made in prior work. As such, our main result is a direct generalization of prior work to accommodate higher-order peer effects. 

We should also discuss the importance, in both our work and the  work we build upon~\cite{Chatterjee07,ghosal2018joint,DDP19}, of estimating the parameters of our model using a {\em single} sample, which stands in contrast to other recent work studying estimation of Ising models and more general Markov Random Fields from  multiple samples; see e.g.~\cite{BreslerGS14,Bresler15,BreslerK16,klivans2017learning,?????}. The importance of estimating from a single simple arises from the applications motivating our work, where it is more common than not that we really only have a single sample of node behavior across the whole network, and  cannot  obtain a fresh independent sample of behavior tomorrow or within a reasonable time-frame.

\paragraph{Techniques.} Towards obtaining Theorem~\ref{thm:informalone}, we encounter several technical challenges. A natural approach is to use our single sample to perform Maximum Likelihood Estimation. However, this approach faces two important challenges. First, it has been shown that the single sample Maximum Likelihood Estimator is not necessarily consistent~\cite{Chatterjee07}. Second, the likelihood function involves the partition function $Z_{\theta,\beta}$, which is generally computationally intractable to compute. In view of these issues, we follow instead the approach followed in prior work. Rather than maximizing the likelihood of the sample, we maximize its {\em pseudolikelihood}, defined as $\prod_i \Pr[y_i~|~\vec{y}_{-i}]$. This concave function of our parameters $\theta$ and $\beta$ is computationally easy to optimize, however we need to show that its maximum is consistent. To argue this we establish two main properties of the log-pseudolikelihood: (i) the log-pseudolikelihood is strongly concave in the neighborhood of its maximum; and (ii)  its gradient at the true model parameters is bounded. As both the Hessian and the gradient of log-pseudolikelihood are functions of the vector of variables $\vec{y}$, which are jointly sampled, to argue (i) and (ii)  we need to control functions of depedent random variables. We do this we use exchangeable pairs,  adapting the technique of ~\cite{chatterjee2016nonlinear}, combined with a parity argument on $G$ and $f$'s partial derivatives. Combined, (i) and (ii) establish the consistency of the Maximum Pseudolikelihood Estimator (MPLE).


%use concentration of measure in Ising models with higher-order interactions combined with a parity argument to establish that 
%We show both properties via concentration results for functions of  dependent random variables. To show that the maximum of the pseudolikelihood is close to the true parameters we use exchangeable pairs, adapting~\cite{chatterjee2016nonlinear}. To show that it is strongly convex we show additional properties of $A$ which are implied by our assumptions. Combining these with a new concentration inequality, we obtain the desired bound. A more complete overview of the approach is presented in Section~\ref{sec:logistic-overview}.

\paragraph{Draft...}
\begin{itemize}
	%\item Graphical models are a rich family of high-dimensional distributions with numerous applications in XYZ fields.
	%\item One of the most important tasks studied on graphical models is that of learning the model using samples. Typically has been studied in the context where we are given access to many samples. (Bresler, Ankur, Klivans, and others)
	%\item However, it might be the case that we are observing people on a network connected by an underlying graphical model and we don't have access to multiple social networks. In such cases we have access to only a single sample from a large model described by a small number of parameters and we would like to do inference in this setting.
	%\item Studied by Chatterjee. Problem with MLE is  both computational and statistical. partition function and not knowing the consistency of MLE.
	\item Pseudo-likelihood estimator. How to prove consistency? Two main steps - Bounding norm of gradient at true parameters, showing strong concavity of log pseudolikelihood. Both steps challenging due to dependence. Chatterjee applied technique of exchangeable pairs for this setting. We adapt his approach.
	%\item Extend his result to models which go beyond pairwise correlations.
	%\item Main technique is in the approach to show strong concavity.
\end{itemize}





\paragraph{Technical Overview:}
\begin{comment}
The estimation algorithms in both Theorem~\ref{thm:logistic} and Theorem~\ref{thm:linear} are instances of Projected Gradient Descent (PGD). In the linear case (Theorem~\ref{thm:linear}, PGD is applied to the negative log-likelihood of the observations $(y_1,\ldots,y_n)$. However, the log-likelihood is not convex, so we perform a re-parametrization of the model, indeed an {\em overparametrization} of the model that renders it convex. Showing strong convexity of the re-parametrized negative log-likelihood requires some mild linear algebra. It has to be established that despite the overparametrization the optimum collapses to the right dimensionality, and can be used to recover the original parameters. A more complete overview of the approach is presented in the beginning of Section~\ref{sec:linear}.

In the logistic case (Theorem~\ref{thm:logistic}), we do not run PGD on the negative log-likelihood but the negative\\ log-{\em pseudo}likelihood. Pseudolikelihood is the product of the conditional probabilities of each response $y_i$, conditioning on all other responses $y_{-i}$. Pseudolikelihood is trivially convex, but we need to establish that is optimum is close to the true parameters and also that it is strongly convex. We show both properties via concentration results for functions of  dependent random variables. To show that the maximum of the pseudolikelihood is close to the true parameters we use exchangeable pairs, adapting~\cite{chatterjee2016nonlinear}. To show that it is strongly convex we show additional properties of $A$ which are implied by our assumptions. Combining these with a new concentration inequality, we obtain the desired bound. A more complete overview of the approach is presented in Section~\ref{sec:logistic-overview}.
\end{comment} 

==> intro_think_older.tex <==
\section{Introduction}
\label{sec:intro}

Did you choose \textcolor{red}{red} rather than \textcolor{blue}{blue} because some inherent attributes of yours biased you towards \textcolor{red}{red}, or because your social environment biased you towards \textcolor{red}{that} color? Of course, the answer is typically ``\textcolor{red}{bo}\textcolor{blue}{th}.'' Indeed, a long literature in econometrics and the social sciences has substantiated the importance of peer effects in network behavior in topics as diverse as criminal activity (see e.g.~\cite{glaeser1996crime}), welfare participation (see e.g.~\cite{bertrand2000network}), school achievement (see e.g.~\cite{sacerdote2001peer}), participation in retirement plans~\cite{duflo2003role}, and obesity (see e.g.~\cite{trogdon2008peer,christakis2013social}).
%A prominent dataset where peer effects have been studied are data collected by the National Longitudinal Study of Adolescent Health, a.k.a.~AddHealth study~\cite{harris2009waves}. This was a major national study of students in grades 7-12, who were asked to name their friends---up to 10, so that friendship networks can be constructed, and answer hundreds of questions about their personal and school life, and it also recorded information such as the age, gender, race, socio-economic background, and health of the students.
Estimating models that combine peer and individual effects to predict behavior in such settings has been challenging; see~e.g.~\cite{manski1993identification,bramoulle2009identification}.

From a modeling perspective, a class of probabilistic models that are commonly used to model behavior in social networks are spin glass models, such as the well-studied Sherrington-Kirkpatrick, Hopfield and Ising models. In these models, a vector of binary behaviors $\vec{y} \in \{-1,1\}^V$ across all nodes of a network $G=(V,E)$ is sampled jointly according to the Gibbs distribution, $p(\vec{y})={1 \over Z} \exp(-{\rm En}(\vec{y}))$, defined by some energy function ${\rm En}(\vec{y})$ of the aggregate behavior, where  ${\rm En}(\cdot)$ is typically defined in terms of both the structure of the network and properties of the nodes. Such models studied originally in Statistical Physics, have found myriad applications in diverse fields, including probability theory, Markov Chain Monte Carlo, Computer Vision, Computational Biology, Game Theory and Social Networks~\cite{LevinPW09,Chatterjee05,Felsenstein04,DaskalakisMR11,GemanG86,Ellison93,MontanariS10}.

Generalizing the classical logistic regression model, we study binary behavior on a social network $G=(V,E)$, whose nodes' behavior depends both on their individual characteristics $\vec{x}_i \in \mathbb{R}^d$, $i \in V$, and the behaviors of the other nodes, according to some measure of the following form:
\begin{align}\Pr[\vec{y}] = {1 \over Z_{\theta,\beta}} \exp\left(\sum_{i=1}^n(\theta^{\rm T} \vec{x}_i) y_i + \beta\cdot f(\vec{y})\right), \label{eq:the model}
\end{align}
where a linear function $\theta^T \vec{x}_i$ of node $i$'s individual characteristics determines the ``external field'' on that node, and some function $f(\vec{y})$ of the nodes' joint behavior expresses what configurations in $\{\pm 1 \}^V$ are encouraged by peer-group effects. Recent works of Chatterjee~\cite{Chatterjee07}, Ghosal and Mukerjee~\cite{ghosal2018joint} and Daskalakis et al.~\cite{DDP19} considered the case where $f$ contains only pair-wise effects, i.e.~the function $f$ is a multilinear function of degree $2$, and the goal of our work is to extend these results to $f$'s with peer effects of higher-order. As such, our models are richer, capturing a much broader range of social interactions, e.g.~settings where nodes belong in various groups, and dislike fragile majorities of behavior in the groups they belong to.

Given a collection $\vec{x}_1,\ldots,\vec{x}_n \in \mathbb{R}^d$ of covariates, some function $f: \{\pm 1\}^V \rightarrow \mathbb{R}$, and a {\em single} sample $\vec{y}$ drawn according to the measure given in~\eqref{eq:the model}, our goal is to output an estimate $(\hat{\theta},\hat{\beta})$ of the true parameters $(\theta,\beta)$.

%\paragraph{Draft...}
%\begin{itemize}
%	%\item Graphical models are a rich family of high-dimensional distributions with numerous applications in XYZ fields.
%	\item One of the most important tasks studied on graphical models is that of learning the model using samples. Typically has been studied in the context where we are given access to many samples. (Bresler, Ankur, Klivans, and others)
%	\item However, it might be the case that we are observing people on a network connected by an underlying graphical model and we don't have access to multiple social networks. In such cases we have access to only a single sample from a large model described by a small number of parameters and we would like to do inference in this setting.
%	\item Studied by Chatterjee. Problem with MLE is  both computational and statistical. partition function and not knowing the consistency of MLE.
%	\item Pseudo-likelihood estimator. How to prove consistency? Two main steps - Bounding norm of gradient at true parameters, showing strong concavity of log pseudolikelihood. Both steps challenging due to dependence. Chatterjee applied technique of exchangeable pairs for this setting. We adapt his approach.
%	\item Extend his result to models which go beyond pairwise correlations.
%	\item Main technique is in the approach to show strong concavity.
%\end{itemize}



\begin{theorem}[Informal] \label{thm:informalone}
Let $G(V,E)$ be a hypergraph with edges of cardinality at least two and at most $m$ and weights $w_{\vec{e}}$. Assume that each vertex has bounded degree (Assumption \ref{eq:bounded}) and the number of edges is large enough (Assumption \ref{eq:lowebounded}). Moreover, assume that true parameters $\theta_0, \beta_0$ and the feature vectors have bounded $\ell_2$ (Assumption \ref{eq:assumption3}). We can compute \textit{from one sample} and  in \textit{polynomial time} an estimator $\tilde{\theta}, \tilde{\beta}$ such that $\norm{(\tilde{\theta},\tilde{\beta})-(\theta_0,\beta_0)}_2$ is
$2^{O(m)} \cdot O\left(\sqrt{\frac{d}{n}}\right)$.
\end{theorem}

\paragraph{Technical Overview:}
\begin{comment}
The estimation algorithms in both Theorem~\ref{thm:logistic} and Theorem~\ref{thm:linear} are instances of Projected Gradient Descent (PGD). In the linear case (Theorem~\ref{thm:linear}, PGD is applied to the negative log-likelihood of the observations $(y_1,\ldots,y_n)$. However, the log-likelihood is not convex, so we perform a re-parametrization of the model, indeed an {\em overparametrization} of the model that renders it convex. Showing strong convexity of the re-parametrized negative log-likelihood requires some mild linear algebra. It has to be established that despite the overparametrization the optimum collapses to the right dimensionality, and can be used to recover the original parameters. A more complete overview of the approach is presented in the beginning of Section~\ref{sec:linear}.

In the logistic case (Theorem~\ref{thm:logistic}), we do not run PGD on the negative log-likelihood but the negative\\ log-{\em pseudo}likelihood. Pseudolikelihood is the product of the conditional probabilities of each response $y_i$, conditioning on all other responses $y_{-i}$. Pseudolikelihood is trivially convex, but we need to establish that is optimum is close to the true parameters and also that it is strongly convex. We show both properties via concentration results for functions of  dependent random variables. To show that the maximum of the pseudolikelihood is close to the true parameters we use exchangeable pairs, adapting~\cite{chatterjee2016nonlinear}. To show that it is strongly convex we show additional properties of $A$ which are implied by our assumptions. Combining these with a new concentration inequality, we obtain the desired bound. A more complete overview of the approach is presented in Section~\ref{sec:logistic-overview}.
\end{comment} 
